Koszulity, supersolvability, and Stirling representations

Supersolvable hyperplane arrangements and matroids are known to give rise to certain Koszul algebras, namely their Orlik-Solomon algebras and graded Varchenko-Gel'fand algebras. We explore how this interacts with group actions, particularly for the braid arrangement and the action of the symmetric group, where the Hilbert functions of the algebras and their Koszul duals are given by Stirling numbers of the first and second kinds, respectively. The corresponding symmetric group representations exhibit branching rules that interpret Stirling number recurrences, which are shown to apply to all supersolvable arrangements. They also enjoy representation stability properties that follow from Koszul duality.

==> tables/old-OS-VG-tables.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{center}
    Representations for deviations $\varphi_i$ for $\OS(\cA_{n-1})$ 
\end{center}
\ytableausetup{boxsize = 0.5em}
%    \centering
    \begin{tabular}{|c|c|c|c|c|c|c}
\hline
 & $\varphi_1$ & $\varphi_2$ & $\varphi_3$ & $\varphi_4$ & $\varphi_5$
 \\
 \hline \hline $\cA_1$ & \ydiagram{2} & & & & \\
 \hline $\cA_2$ & \ydiagram{2,1} + \ydiagram{3} & \ydiagram{1,1,1} & \ydiagram{2,1} & \ydiagram{1,1,1} + \ydiagram{2,1} & $3\cdot \ydiagram{1,1,1} + 6\cdot \ydiagram{2,1} + 3\cdot \ydiagram{3}$\\ \hline $\cA_3$ & \ydiagram{2,2} + \ydiagram{3,1} + \ydiagram{4} & $\ydiagram{1,1,1,1} + \ydiagram{2,1,1}$ & $\ydiagram{2,1,1} + 2\cdot \ydiagram{2,2} + \ydiagram{3,1}$ & $2\cdot \ydiagram{1,1,1,1} + 3\cdot \ydiagram{2,1,1}$ & $13\cdot\ydiagram{1,1,1,1} + 31 \cdot \ydiagram{2,1,1} + 26 \cdot \ydiagram{2,2}$ \\
 & & & & $+ 2\cdot \ydiagram{2,2} + 2\cdot \ydiagram{3,1}$ & $+31\cdot \ydiagram{3,1} + 13\cdot \ydiagram{4}$ \\
 \hline $\cA_4$ & \ydiagram{3,2}+\ydiagram{4,1}& \ydiagram{2,1,1,1} + \ydiagram{3,1,1} & $2\cdot \ydiagram{2,2,1} + \ydiagram{3,1,1}$ & $\ydiagram{1,1,1,1,1} 
+ 3\cdot\ydiagram{2,1,1,1} + 3\cdot \ydiagram{2,2,1}$ & $15\cdot\ydiagram{1,1,1,1,1} + 
 58\cdot \ydiagram{2,1,1,1} + 80\cdot \ydiagram{2,2,1}$
 \\
 & +\ydiagram{4} & & $ + 2\cdot \ydiagram{3,2} + \ydiagram{4,1}$ & $+5\cdot \ydiagram{3,1,1} + 3\cdot \ydiagram{3,2}$ & $+90\cdot \ydiagram{3,1,1} + 85\cdot \ydiagram{3,2}$ \\
 & & & & $+ 2\cdot \ydiagram{4,1}$ & $ + 69\cdot \ydiagram{4,1} + 20\cdot \ydiagram{5}$ \\ \hline
 $\cA_5$ & \ydiagram{4,2} + \ydiagram{5,1} & \ydiagram{3,1,1,1}  + \ydiagram{4,1,1} & $\ydiagram{2,2,2} + 2\cdot\ydiagram{3,2,1}$ & $\ydiagram{2,1,1,1,1} +\ydiagram{2,2,1,1} + \ydiagram{2,2,2}$ & \\
 & +\ydiagram{6} & & $\ydiagram{4,1,1} + 2\cdot \ydiagram{4,2}$ & $4\cdot \ydiagram{3,1,1,1} + 5\cdot\ydiagram{3,2,1} + \ydiagram{3,3}$ & \\
 & & & \ydiagram{5,1} & $5\cdot \ydiagram{4,1,1} + 3\cdot \ydiagram{4,2}$ &\\ & & & &  $+2\cdot\ydiagram{5,1}$ & \\ \hline
\end{tabular}

%%%%%%
\begin{center}
    Representations for deviations $\varphi_i$ for $\VG(\cA_{n-1})$ 
\end{center}
\ytableausetup{boxsize = 0.5em}
% \centering
    \begin{tabular}{|c|c|c|c|c|c|c}
\hline
 & $\varphi_1$ & $\varphi_2$ & $\varphi_3$ & $\varphi_4$ & $\varphi_5$
 \\ \hline \hline 
 $\cA_1$ & \ydiagram{1,1} & \ydiagram{2} & & & \\ \hline
 $\cA_2$ & \ydiagram{1,1,1} + \ydiagram{2,1} & $\ydiagram{2,1} + 2\cdot \ydiagram{3}$ & \ydiagram{2,1} & \ydiagram{1,1,1} + \ydiagram{2,1}  & $\ydiagram{1,1,1} + 2\cdot \ydiagram{2,1} + \ydiagram{3}$\\ \hline
 $\cA_3$ & \ydiagram{2,1,1} + \ydiagram{3,1} & $\ydiagram{2,2} + 2\cdot \ydiagram{3,1} + 2\cdot \ydiagram{4}$ & $\ydiagram{2,1,1} + 2\cdot \ydiagram{2,2} + \ydiagram{3,1}$ & $\ydiagram{1,1,1,1}+ 4\cdot \ydiagram{2,1,1}$ & $2\cdot\ydiagram{1,1,1,1} + 7\cdot\ydiagram{2,1,1} + 4\cdot \ydiagram{2,2}$ \\
 & & & & $+\ydiagram{2,2} + 2\cdot \ydiagram{3,1}$ & $+7\cdot \ydiagram{3,1} + 2\cdot\ydiagram{4}$\\ \hline
 $\cA_4$ & \ydiagram{3,1,1} + \ydiagram{4,1} & $2\cdot\ydiagram{3,2} + 2\cdot \ydiagram{4,1}$ & $2\cdot\ydiagram{2,2,1} + \ydiagram{3,1,1}$ & $3\cdot\ydiagram{2,1,1,1} + 3\cdot \ydiagram{2,2,1}$ & $\ydiagram{1,1,1,1,1} + 8 \cdot \ydiagram{2,1,1,1} + 10\cdot \ydiagram{2,2,1}$ \\&&$2\cdot\ydiagram{5}$& $2\cdot\ydiagram{3,2} + \ydiagram{4,1}$ & $6\cdot \ydiagram{3,1,1} + 2\cdot\ydiagram{3,2}$ & $13\cdot \ydiagram{3,1,1} + 11\cdot\ydiagram{3,2}$ \\ & & & & $+2\cdot\ydiagram{2,2,1}$ & $+2\cdot\ydiagram{5}$ \\ \hline
 $\cA_5$ & \ydiagram{4,1,1} + \ydiagram{5,1} & $\ydiagram{3,3} + 2\cdot \ydiagram{4,2}$ & $\ydiagram{2,2,2} + 2\cdot \ydiagram{3,2,1}$ & $2\cdot\ydiagram{2,2,1,1} + 4\cdot \ydiagram{3,1,1,1}$ & \\
 &&$2\cdot\ydiagram{5,1} + 2\cdot\ydiagram{5}$ & $\ydiagram{4,1,1} + 2\cdot\ydiagram{4,2}$ & $+5\cdot\ydiagram{3,2,1} + \ydiagram{3,3}$ & \\
&&&\ydiagram{5,1}&$6\cdot\ydiagram{4,1,1} + 2\cdot\ydiagram{4,2}$ & \\
 &&&& $2\cdot\ydiagram{5,1}$&\\ \hline
 \end{tabular}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vic{I agree.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{center}
    Representations $\mathcal{S}_\OS(n,k) = A^!(k+1)_{n-k}$ 
\end{center}
\ytableausetup{boxsize = 0.5em}
%    \centering
    \begin{tabular}{|c|c|c|c|c|c|c}
\hline
$n/k$ & 0 & 1 & 2 & 3 & 4\\
\hline \hline 0 & $1\cdot \ydiagram{1}$ &  & & &\\
\hline 1 & & $1\cdot \ydiagram{2}$ & & &\\
\hline 2 & & $1\cdot \ydiagram{2}$ & $1\cdot \ydiagram{3}$ & & \\
\hline 3 & & $1\cdot \ydiagram{2}$ & $1\cdot \ydiagram{3}, \; 1\cdot \ydiagram{2,1}$ & $1\cdot \ydiagram{4}$ & \\
\hline 4 & & $1\cdot \ydiagram{2}$ & $2\cdot \ydiagram{3}, \; 2\cdot \ydiagram{2,1}, \; 1\cdot \ydiagram{1,1,1} $ & $1\cdot \ydiagram{2,2}, \; 1\cdot \ydiagram{3,1}, \; 1\cdot \ydiagram{4} $ & $1\cdot \ydiagram{5}$ \\
\hline 5 & & $1\cdot \ydiagram{2}$ & $3\cdot \ydiagram{3}, \; 5\cdot \ydiagram{2,1}, \; 2\cdot \ydiagram{1,1,1}$ & $1\cdot \ydiagram{1,1,1,1}, \; 2\cdot \ydiagram{2,1,1}, \; 3\cdot \ydiagram{2,2} $ & $1\cdot \ydiagram{3,2}, \; 1\cdot \ydiagram{4,1}, \; 1\cdot \ydiagram{5}$\\
 & & & & $3\cdot \ydiagram{3,1}, \; 3\cdot \ydiagram{4}$ &  \\
\hline 6 & & $1\cdot \ydiagram{2}$ & $6\cdot \ydiagram{3}, \; 10\cdot \ydiagram{2,1}, \; 5\cdot \ydiagram{1,1,1}$ & $4\cdot \ydiagram{1,1,1,1}, \; 9\cdot \ydiagram{2,1,1}, \; 10\cdot \ydiagram{2,2}, \;$ & $1\cdot \ydiagram{2,1,1,1}, \; 2\cdot \ydiagram{2,2,1}, \; 2\cdot \ydiagram{3,1,1}, \;$ \\ & & & & $11\cdot \ydiagram{3,1}, \; 6 \ydiagram{4}$ & $4\cdot\ydiagram{3,2}, \; 4\cdot \ydiagram{4,1}, \; 3\cdot \ydiagram{5}$ \\
\hline 7 & & $1\cdot \ydiagram{2}$ & $11\cdot \ydiagram{3}, \; 21\cdot \ydiagram{2,1}, \; 10\cdot \ydiagram{1,1,1}$ & $14\cdot \ydiagram{1,1,1,1}, \; 34\cdot \ydiagram{2,1,1}, \; 30\cdot \ydiagram{2,2}, \;$ & $2\cdot\ydiagram{1,1,1,1,1}, \; 8\cdot \ydiagram{2,1,1,1}, \; 13\cdot \ydiagram{2,2,1}, \; 15\cdot \ydiagram{3,1,1}, \;$ \\ & & & & $36\cdot \ydiagram{3,1}, \; 17 \ydiagram{4}$ & $18\cdot\ydiagram{3,2}, \; 16\cdot \ydiagram{4,1}, \; 7\cdot \ydiagram{5}$ \\\hline 8 & & $1\cdot \ydiagram{2}$ & $22\cdot \ydiagram{3}, \; 42\cdot \ydiagram{2,1}, \; 21\cdot \ydiagram{1,1,1}$ & $44\cdot \ydiagram{1,1,1,1}, \; 114\cdot \ydiagram{2,1,1}, \; 91\cdot \ydiagram{2,2}, \;$ & $12\cdot\ydiagram{1,1,1,1,1}, \; 48\cdot \ydiagram{2,1,1,1}, \; 68\cdot \ydiagram{2,2,1}, \; 80\cdot \ydiagram{3,1,1}, \;$ \\ & & & & $117\cdot \ydiagram{3,1}, \; 47 \ydiagram{4}$ & $78\cdot\ydiagram{3,2}, \; 66\cdot \ydiagram{4,1}, \; 23\cdot \ydiagram{5}$\\ \hline 
    \end{tabular}
% \caption{Representations $\cS(n,k)$ corresponding to graded pieces of $\OS(\cB_n)^!$ }
% \label{tab:Stirling-2-reps-OS}

%%%%%%

\begin{center}
    Representations $\mathcal{S}_\VG(n,k) = A^!(k+1)_{n-k}$ 
\end{center}
%    \centering
    \begin{tabular}{|c|c|c|c|c|c|c}
\hline
$n/k$ & 0 & 1 & 2 & 3 & 4\\
\hline \hline 0 & $1\cdot \ydiagram{1}$ &  & & &\\
\hline 1 & & $1\cdot \ydiagram{2}$ & & &\\
\hline 2 & & $1\cdot \ydiagram{1,1}$ & $1\cdot \ydiagram{3}$ & & \\
\hline 3 & & $1\cdot \ydiagram{2}$ & $1\cdot \ydiagram{1,1,1}, \; 1\cdot \ydiagram{2,1}$ & $1\cdot \ydiagram{4}$ & \\
\hline 4 & & $1\cdot \ydiagram{1,1}$ & $2\cdot \ydiagram{3}, \; 2\cdot \ydiagram{2,1}, \; 1\cdot \ydiagram{1,1,1} $ & $1\cdot \ydiagram{2,1,1}, \; 1\cdot \ydiagram{3,1}$ & $1\cdot \ydiagram{5}$ \\
\hline 5 & & $1\cdot \ydiagram{2}$ & $2\cdot \ydiagram{3}, \; 5\cdot \ydiagram{2,1}, \; 3\cdot \ydiagram{1,1,1}$ & $1\cdot \ydiagram{1,1,1,1}, \; 3\cdot \ydiagram{2,1,1}, \; 2\cdot \ydiagram{2,2},$ & $1\cdot \ydiagram{3,1,1}, \; 1\cdot \ydiagram{4,1}$\\
& & & & $3\cdot \ydiagram{3,1}, \; 2\cdot\ydiagram{4}$ & \\
\hline 6 & & $1\cdot \ydiagram{1,1}$ & $6\cdot \ydiagram{3}, \; 10\cdot \ydiagram{2,1}, \; 5\cdot \ydiagram{1,1,1}$ & $4\cdot \ydiagram{1,1,1,1}, \; 11\cdot \ydiagram{2,1,1}, \; 8\cdot \ydiagram{2,2}, \;$ & $2\cdot \ydiagram{2,1,1,1}, \; 2\cdot \ydiagram{2,2,1}, \; 3\cdot \ydiagram{3,1,1}, \;$ \\ & & & & $11\cdot \ydiagram{3,1}, \; 4 \ydiagram{4}$ & $3\cdot\ydiagram{3,2}, \; 3\cdot \ydiagram{4,1}, \; 2\cdot \ydiagram{5}$ \\ 
\hline 7 & & $1\cdot \ydiagram{2}$ & $10\cdot \ydiagram{3}, \; 21\cdot \ydiagram{2,1}, \; 11\cdot \ydiagram{1,1,1}$ & $12\cdot \ydiagram{1,1,1,1}, \; 38\cdot \ydiagram{2,1,1}, \; 24\cdot \ydiagram{2,2}, \;$ & $3\cdot\ydiagram{1,1,1,1,1}, \; 10\cdot \ydiagram{2,1,1,1}, \; 14\cdot \ydiagram{2,2,1}, \; 17\cdot \ydiagram{3,1,1}, \;$ \\ & & & & $38\cdot \ydiagram{3,1}, \; 13 \ydiagram{4}$ & $15\cdot\ydiagram{3,2}, \; 14\cdot \ydiagram{4,1}, \; 4\cdot \ydiagram{5}$ \\
\hline 8 & & $1\cdot \ydiagram{1,1}$ & $22\cdot \ydiagram{3}, \; 42\cdot \ydiagram{2,1}, \; 21\cdot \ydiagram{1,1,1}$ & $40\cdot \ydiagram{1,1,1,1}, \; 121\cdot \ydiagram{2,1,1}, \; 80\cdot \ydiagram{2,2}, \;$ & $12\cdot\ydiagram{1,1,1,1,1}, \; 54\cdot \ydiagram{2,1,1,1}, \; 68\cdot \ydiagram{2,2,1}, \; 86\cdot \ydiagram{3,1,1}, \;$ \\ & & & & $121\cdot \ydiagram{3,1}, \; 40 \ydiagram{4}$ & $72\cdot\ydiagram{3,2}, \; 60\cdot \ydiagram{4,1}, \; 17\cdot \ydiagram{5}$\\ \hline
    \end{tabular}
% \caption{Representations $\cS(n,k)$ corresponding to graded pieces of $\VG(\cB_n)^!$ }
% \label{tab:Stirling-2-reps-VG}


